Correspondence Learning via Linearly-invariant Embedding

In this paper, we propose a fully differentiable pipeline for estimating accurate dense correspondences between 3D point clouds. The proposed pipeline is an extension and a generalization of the functional maps framework. However, instead of using the Laplace-Beltrami eigenfunctions as done in virtually all previous works in this domain, we demonstrate that learning the basis from data can both improve robustness and lead to better accuracy in challenging settings. We interpret the basis as a learned embedding into a higher dimensional space. Following the functional map paradigm the optimal transformation in this embedding space must be linear and we propose a separate architecture aimed at estimating the transformation by learning optimal descriptor functions. This leads to the first end-to-end trainable functional map-based correspondence approach in which both the basis and the descriptors are learned from data. Interestingly, we also observe that learning a \emph{canonical} embedding leads to worse results, suggesting that leaving an extra linear degree of freedom to the embedding network gives it more robustness, thereby also shedding light onto the success of previous methods. Finally, we demonstrate that our approach achieves state-of-the-art results in challenging non-rigid 3D point cloud correspondence applications.

==> figures/figure_phiM.tex <==

\begin{figure}[!t]
\centering

  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{c c c c c c c c c c}
\hspace{-0.3cm}
  
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_01.png}
  \put(12,-9){\footnotesize{$\Phi_M1$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_02.png}
  \put(12,-9){\footnotesize{$\Phi_M2$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_03.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M3$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_04.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M4$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_05.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M5$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_06.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M6$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_07.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M7$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_08.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M8$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_09.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M9$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_10.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M10$}}}
   \end{overpic}
\end{minipage}
\\

\vspace{1mm}

\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_11.png}
  \put(12,-9){\footnotesize{$\Phi_M11$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_12.png}
  \put(12,-9){\footnotesize{$\Phi_M12$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_13.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M13$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_14.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M14$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_15.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M15$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_16.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M16$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_17.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M17$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_18.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M18$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_19.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M19$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiM_20.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_M20$}}}
   \end{overpic}
\end{minipage}
\end{tabular}
\end{figure}

==> figures/figure_phiN.tex <==

\begin{figure}[!t]
\centering

  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{c c c c c c c c c c}
\hspace{-0.3cm}
  
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_01.png}
  \put(12,-9){\footnotesize{$\Phi_N1$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_02.png}
  \put(12,-9){\footnotesize{$\Phi_N2$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_03.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N3$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_04.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N4$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_05.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N5$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_06.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N6$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_07.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N7$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_08.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N8$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_09.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N9$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_10.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N10$}}}
   \end{overpic}
\end{minipage}
\\

\vspace{1mm}

\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_11.png}
  \put(12,-9){\footnotesize{$\Phi_N11$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_12.png}
  \put(12,-9){\footnotesize{$\Phi_N12$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_13.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N13$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_14.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N14$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_15.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N15$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_16.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N16$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_17.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N17$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_18.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N18$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_19.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N19$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_ori_20.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_N20$}}}
   \end{overpic}
\end{minipage}
\end{tabular}
\end{figure}

==> figures/figure_phiN_transf.tex <==

\begin{figure}[!t]
\centering

  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{c c c c c c c c c c}
\hspace{-0.3cm}
  
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_01.png}
  \put(12,-9){\footnotesize{$\Phi_NA_{NM}1$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_02.png}
  \put(12,-9){\footnotesize{$\Phi_NA_{NM}2$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_03.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}3$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_04.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}4$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_05.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}5$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_06.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}6$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_07.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}7$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_08.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}8$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_09.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}9$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_10.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}10$}}}
   \end{overpic}
\end{minipage}
\\

\vspace{1mm}

\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_11.png}
  \put(12,-9){\footnotesize{$\Phi_NA_{NM}11$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_12.png}
  \put(12,-9){\footnotesize{$\Phi_NA_{NM}12$}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_13.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}13$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_14.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}14$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_15.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}15$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_16.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}16$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_17.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}17$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_18.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}18$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_19.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}19$}}}
   \end{overpic}
\end{minipage}
&
\begin{minipage}{0.1\linewidth}
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.93\linewidth]{./figures/basis/phiN_20.png}
  \put(12,-9){\footnotesize{\textbf{$\Phi_NA_{NM}20$}}}
   \end{overpic}
\end{minipage}
\end{tabular}
\end{figure}

==> sections/analysis.tex <==
\section{Insights, relations and strengths}
\label{sec:insights}
\subsection{Relation with the universal embedding pipeline}
The proposed method can be also seen as a generalization of the universal embedding problem. The solution of the universal embedding problem is a multidimensional embedding where similar points from different objects are mapped nearby and conversely different ones are mapped farther. No transformation are required and the correspondence can be computed directly as a nearest neighbour search between the embeddings.
Despite this approach can be general and applicable to different representations it is based on a quite strong claim, that is to find a unique representations for different shapes also when these undergo to rigid and non rigid deformations.
Our approach is more general in the sense that, in addition to the embedding we consider the presence of a linear transformation which should be applied to obtain a similar embedding from two different shapes.
To compare with the universal embedding we learn a possible universal embedding with the loss \ref{eq:loss_spatial} without requiring an optimal transformation between the embeddings (i.e. considering the identity as linear transformation).
As we show in section \ref{sec:results}, our approach outperform this universal embedding solution in all the scenarios we considered.

\subsection{Linear Map for Aligning Embeddings}
\label{sec:alignment}
Given two embeddings $\Phi_{\Y}, \Phi_{\X}$ and a correspondence encoded by the matrix $\Pi_{\X\Y}$ we would like to find a linear transformation $A_{\X\Y}$ that aligns these embeddings.

From equation \ref{eq:nnassignment} we can derive that we are looking for the linear transformation $A_{\X\Y}$ that verifies:
%
\begin{align}
    \argmin_{A_{\X\Y}} \| \Phi_{\X} A_{\X\Y} - \Pi_{\X\Y} \Phi_{\Y}\|_2,
\end{align}
from which the solution is given by:
\begin{align}
    A_{\X\Y} = \Phi_{\X}^{\dagger}(\Pi_{\X\Y} \Phi_{\Y})
\end{align}
Recall that a functional map induced by $\Pi_{\X\Y}$ is defined as the matrix that minimizes:
\begin{align}
    \argmin_{C_{\Y\X}} \| C_{\Y\X}\Phi_{\X}^{\top}  - (\Pi_{\X\Y} \Phi_{\Y})^{\top}\|_2,
\end{align}
for which the solution is given by:
\begin{align}
C_{\Y\X} = \left(\Phi_{\X} ^{\dagger} \Pi_{\X\Y} \Phi_{\Y}\right)^{\top}
\end{align}
Therefore, we can write: $A_{\X\Y} = C_{\Y\X}^{\top}$.

This provides an explicit connection between the functional map and the linear transformation that we are optimizing for.
From the previous discussion, one can conclude that $A_{\X\Y}$ is the transpose of the functional map inverse. Formally, the transpose is also the \emph{map adjoint.} See \cite{huang2017adjoint} for an in-depth discussion of functional map adjoints. 

One advantage of the adjoint is that it can be used to map \emph{distributions} and not just functions. 
In other words, unlike a functional map, the functional map adjoint always maps delta functions to delta functions. For this reason, despite the strong relation with functional maps, the adjoint is better suited for estimating the correspondence.  

\subsection{Strengths}
Learning a new embedding and a new set of probe functions we overcome the main limitation of the functional maps framework.
Our embedding is directly computed on the natural embedding and does not require any approximation of the underlying surface. For this reason it is suited also for point clouds and provides more stable performance than the spectral embedding on less structured input. 
Moreover, the independence from the global representation of the surface and the direct encoding of each singular point enable our pipeline to achieve accurate results also for noisy, partial and for the extreme fragmented cases as proved in section \ref{sec:results}.
Finally, the learned embedding does not own any additional property that is usually by the spectral embedding. The different dimensions of the learned embedding are indeed not orthonormal and can not be ordered in a proper way. Additional properties can be added modifying the loss in the equation \ref{eq:loss_spatial}. In this paper we only present one version but the proposed framework could be potentially extended to other version that could be better suited for specific applications.

% limits of the probe functions
The learned probe functions are informative enough to lead the optimization of the linear transformation. Our probe functions behave coherently on different shapes without requiring any additional supervision in the test phase enabling real applications.

The possible data on which the proposed pipeline can be applied are thus wider than the ones that can be processed by the standard functional maps but are not limited to shapes.
We believe that our method can be applied without additional modifications to graphs, texts and any other data that can be described through a vector-space representation. We claim that the generality of the proposed method paves the way to further investigations in several scenario, and we leave these explorations as future work. 


==> sections/figure.tex <==
\begin{figure}[!t]
\centering
  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{c c c c c c c c}



        \multicolumn{3}{c}{ 
    \hspace{1cm}
    
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.5\linewidth]{./figures/legend.png}

  \end{overpic}
  
  }\\   

& 
\multicolumn{2}{c}{ 



\begin{minipage}{0.15\linewidth} 
\small
\centering



    \begin{tabular}{|l|c|c|}
    
    
    \hline
    
    & noNoise & Noise \\
    \hline
    \textbf{our}    & \textbf{5.4e-2} &   \textbf{6.6e-2} \\
    GFM             & 2.9e-1 & 3.4e-1 \\
    uni             & 7.5e-2 & 8.5e-2 \\
    3DC             &  7.0e-2 & 7.3e-2  \\
    FMAP            & 1.3e-1  & 1.4e-1 \\
    FMAP+Z        & 1.1e-1  & 1.3e-1 \\
    GFM+Z         & 3.1e-1 &  3.8e-1\\
    \hline
    \end{tabular}
    
    \hspace{-8cm}
        
    \begin{tabular}{c|c}
    \centering
    \hspace{-1.3cm}
    
    \input{./figures/PC_000_new.tikz} & 
    \hspace{-0.15cm}
    \input{./figures/PC_001_new.tikz} 
    \end{tabular}
    
 \end{minipage}}
    &        
%   \begin{minipage}{0.15\linewidth} 
%     \input{./figures/PC_000_new.tikz}
%     \input{./figures/PC_001_new.tikz}
%    \end{minipage}%
%    &
\hspace{-1.5cm}

      \begin{minipage}{0.13\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_N1.png}
    \put(50,105){\footnotesize{N}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_N1.png}
  \end{overpic}
   
    \end{minipage}%
    
     &
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_gt1.png}
    \put(18,103){\footnotesize{GT}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_gt1.png}

  \end{overpic}
   
    \end{minipage}%
    
        &
     
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_my1.png}
    \put(15,103){\footnotesize{\textbf{OUR}}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_my1.png}
  \end{overpic}
   
    \end{minipage}%
    
        &
        
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_3DC1.png}
\put(15,103){\footnotesize{3DC}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_3DC1.png}

  \end{overpic}

    \end{minipage}%
    
         &
        
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_nic1.png}
\put(10,103){\footnotesize{GFMAP}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_nic1.png}

  \end{overpic}
   
    \end{minipage} 

    

    
  \end{tabular}
  
\caption{\label{fig:pointclouds}
 On the left, the evaluation in the accuracy of the correspondence for point clouds generated from the FAUST dataset without or with additional noise, with cumulative error curves. On the right, a qualitative example.
}

 \end{figure}
 
 

% \begin{figure}[!t]
% \centering
%   \setlength{\tabcolsep}{0pt}
%   \begin{tabular}{c c c c c}
  
%   \vspace{0cm}
%       &
%             \begin{minipage}{0.3\linewidth} 
%      \input{./figures/PC_000.tikz}
%     \end{minipage}%
    
    
%       &

%       \begin{minipage}{0.3\linewidth} 
%      \input{./figures/PC_001.tikz}
%     \end{minipage}%
    
%     &
    
%     \begin{minipage}{0.3\linewidth} 
%     \input{./figures/PC_002.tikz}
%     \end{minipage}% 
   
%   &
   
%       \begin{minipage}{0.3\linewidth} 
%     \input{./figures/PC_003.tikz}
%     \end{minipage}% 
%     \vspace{0cm}
    
%   \end{tabular}
  
% \caption{\label{fig:Pointclouds}
% Pointclouds curves
% }

% \end{figure}

==> sections/test.tex <==
\begin{figure}[!t]
\centering
  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{c c c c c c c c}



        \multicolumn{3}{c}{ 
    \hspace{1cm}
    
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.5\linewidth]{./figures/legend.png}

  \end{overpic}
  
  }\\   

& 
\multicolumn{2}{c}{ 



\begin{minipage}{0.15\linewidth} 
\small
\centering



    \begin{tabular}{|l|c|c|}
    
    
    \hline
    
    & noNoise & Noise \\
    \hline
    \textbf{our}    & \textbf{5.4e-2} &   \textbf{6.6e-2} \\
    GFM             & 2.9e-1 & 3.4e-1 \\
    uni             & 7.5e-2 & 8.5e-2 \\
    3DC             &  7.0e-2 & 7.3e-2  \\
    FMAP            & 1.3e-1  & 1.4e-1 \\
    FMAP+Z        & 1.1e-1  & 1.3e-1 \\
    GFM+Z         & 3.1e-1 &  3.8e-1\\
    \hline
    \end{tabular}
    
    \hspace{-8cm}
        
    \begin{tabular}{c|c}
    \centering
    \hspace{-1.3cm}
    
    \input{./figures/PC_000_new.tikz} & 
    \hspace{-0.15cm}
    \input{./figures/PC_001_new.tikz} 
    \end{tabular}
    
 \end{minipage}}
    &        
%   \begin{minipage}{0.15\linewidth} 
%     \input{./figures/PC_000_new.tikz}
%     \input{./figures/PC_001_new.tikz}
%    \end{minipage}%
%    &
\hspace{-1.5cm}

      \begin{minipage}{0.13\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_N1.png}
    \put(50,105){\footnotesize{N}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_N1.png}
  \end{overpic}
   
    \end{minipage}%
    
     &
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_gt1.png}
    \put(18,103){\footnotesize{GT}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_gt1.png}

  \end{overpic}
   
    \end{minipage}%
    
        &
     
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_my1.png}
    \put(15,103){\footnotesize{\textbf{OUR}}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_my1.png}
  \end{overpic}
   
    \end{minipage}%
    
        &
        
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_3DC1.png}
\put(15,103){\footnotesize{3DC}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_3DC1.png}

  \end{overpic}

    \end{minipage}%
    
         &
        
      \begin{minipage}{0.1\linewidth} 
     \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/000_M_nic1.png}
\put(10,103){\footnotesize{GFMAP}}
  \end{overpic}
     
 \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./figures/PC_final/001_M_nic1.png}

  \end{overpic}
   
    \end{minipage} 

    

    
  \end{tabular}
  
\caption{\label{fig:pointclouds}
 On the left, the evaluation in the accuracy of the correspondence for point clouds generated from the FAUST dataset without or with additional noise, with cumulative error curves. On the right, a qualitative example.
}

 \end{figure}
 
 

% \begin{figure}[!t]
% \centering
%   \setlength{\tabcolsep}{0pt}
%   \begin{tabular}{c c c c c}
  
%   \vspace{0cm}
%       &
%             \begin{minipage}{0.3\linewidth} 
%      \input{./figures/PC_000.tikz}
%     \end{minipage}%
    
    
%       &

%       \begin{minipage}{0.3\linewidth} 
%      \input{./figures/PC_001.tikz}
%     \end{minipage}%
    
%     &
    
%     \begin{minipage}{0.3\linewidth} 
%     \input{./figures/PC_002.tikz}
%     \end{minipage}% 
   
%   &
   
%       \begin{minipage}{0.3\linewidth} 
%     \input{./figures/PC_003.tikz}
%     \end{minipage}% 
%     \vspace{0cm}
    
%   \end{tabular}
  
% \caption{\label{fig:Pointclouds}
% Pointclouds curves
% }

% \end{figure}
